Parameterized Synthesis with Safety Properties

Parameterized synthesis offers a solution to the problem of constructing correct and verified controllers for parameterized systems. Such systems occur naturally in practice (e.g., in the form of distributed protocols where the amount of processes is often unknown at design time and the protocol must work regardless of the number of processes). In this paper, we present a novel learning based approach to the synthesis of reactive controllers for parameterized systems from safety specifications. We use the framework of regular model checking to model the synthesis problem as an infinite-duration two-player game and show how one can utilize Angluin's well-known L* algorithm to learn correct-by-design controllers. This approach results in a synthesis procedure that is conceptually simpler than existing synthesis methods with a completeness guarantee, whenever a winning strategy can be expressed by a regular set. We have implemented our algorithm in a tool called L*-PSynth and have demonstrated its performance on a range of benchmarks, including robotic motion planning and distributed protocols. Despite the simplicity of L*-PSynth it competes well against (and in many cases even outperforms) the state-of-the-art tools for synthesizing parameterized systems.

==> lstar-chihduo.tex <==
\begin{algorithm}[h]
    \DontPrintSemicolon
	\KwIn{A teacher answers $Mem(w)$ and $Eq(H)$ about a target regular language $R$ and the initial observation table $(S,E,T)$.}
	\Repeat{$Eq(H)=``yes"$}{
	\While{$(S,E,T)$ is not closed}{
		Find a pair $(x,a)\in S\times \Sigma$ such that $\forall y\in S: \mathit{row}_E(xa)\neq \mathit{row}_E(y)$.
		Extend $S$ to $S\cup \{xa\}$ and update $T$ using membership queries accordingly\;
	}
	Build a candidate DFA $H= (S, \Sigma, \delta, \epsilon, F)$, where $\delta=\{(s,a,s')\mid s,s'\in S \wedge \mathit{row}_E(sa)=\mathit{row}_E(s)\}$, the empty string $\epsilon$ is the initial state, and $F=\{s\mid T(s)=\top \wedge s\in S \}$\;
	\uIf{$Eq(H)=(\mbox{``no''}, w)$, where $w \in L(H) \ominus R$}{
		Analyze $w$ and add a suffix of $w$ to $E$}
	}
	\KwRet $H$ as the minimal DFA for $R$\;
	\caption{The improved $L^*$ algorithm by Rivest and Schapire}\label{alg:lstar}
\end{algorithm}

==> lstar-oliver.tex <==
\begin{algorithm}[h]
	\DontPrintSemicolon
	\KwIn{A teacher answers membership and equivalence queries about a regular target language $R$}
	\BlankLine
	
	{Initialize an empty observation table $O =(S,E,T)$ with $S = \{\epsilon\}$ and $E = \{\epsilon\}$}
	
	
	\BlankLine
	{Fill the mapping $T$ by answering membership queries for all $w \in \Sigma$}
	\BlankLine
	\Repeat{the teacher replies ``yes'' to an equivalence query}{
		\While{O is not closed or not consistent}
		{\uIf{If O is not closed}{
				Find $x \in S$ and $a \in \Sigma$ such that $\forall y \in S: row_E(xa) \neq row_E(y)$. \;
				$S \leftarrow S \cup \{xa\}$\;
				update T using membership queries\;
			}
			\uElseIf{O is not consistent}{
				Find $x,y \in S, a \in \Sigma$ and $w \in E$ such that \;
				$row_E(x) = row_E(y)$ but $T(xaw) \neq T(yaw)$ \;
				$E \leftarrow E \cup \{aw\}$ \;
				update T using membership queries\;
		}}
		{Construct DFA $\mathcal{A}_h = (S,\Sigma,\delta,\epsilon, F)$, where \;
			$\delta = \{(s,a,s') \mid s,s' \in S \wedge row_E(sa) = row_E(s)\},$ \;
			the empty word $\epsilon$ is the initial state and \;
			$F = \{s \mid T(s) = 1 \wedge s \in S\}$\;}
		{Perform an equivalence query with $\mathcal{A}_h$.} \;
		\uIf{teacher replies with a counterexample $w$}{
			$S \leftarrow S \cup Pref(\{w\})$\;
			update T using membership queries\;
		}
	}{\textbf{return} $\mathcal{A}_h$}
	
	\caption{Angluin's algorithm} \label{alg:lstar}
\end{algorithm}

